Vector Space of Feynman Integrals and Multivariate Intersection Numbers

Feynman integrals obey linear relations governed by intersection numbers, which act as scalar products between vector spaces. We present a general algorithm for constructing multivariate intersection numbers relevant to Feynman integrals, and show for the first time how they can be used to solve the problem of integral reduction to a basis of master integrals by projections, and to directly derive functional equations fulfilled by the latter. We apply it to the derivation of contiguity relations for special functions admitting multi-fold integral representations, and to the decomposition of a few Feynman integrals at one- and two-loops, as first steps towards potential applications to generic multi-loop integrals.

==> Bubble-box.tex <==
\section{\label{sec:massless-bubblebox}Appendix B: Massless Bubble-Box}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.12\textwidth]{bubble_box_zlabels_momenta2.png}
    \caption{Massless bubble-box with massless external legs\\
    ($p_{i}$ with $p_{i}^{2}=0$, for $i=1,2,3,4$). The invariants are $s=(p_{1}+p_{2})^2$ and $t=(p_{2}+p_{3})^2$.}
    \label{fig:Massles_BubbleBox}
\end{figure}

We consider the massless bubble-box diagram at two loops, shown in  Fig.~\ref{fig:Massles_BubbleBox}, which is a sub-graph of the 7-denominator four-point diagram appearing in Fig.~\ref{fig:otherdiagrams}.
%The external (incoming) momenta are denoted $p_{i}$ with $p_{i}^{2}=0$ for $i=1,2,3,4$. We define the kinematic invariants to be $s=(p_{1}+p_{2})^2$, and $t=(p_{2}+p_{3})^2$.
%MOVE TO FIGURE/APPENDIX
%The denominators are given by:
%\begin{align}
%& z_{1}=\left(k_2-p_1-p_2-p_3\right){}^2 \, , \quad  z_{2}=\left(k_2-p_2-p_3\right){}^2  \, ,\nonumber\\
%& z_{3}=\left(k_2-p_3\right){}^2  \, , \quad z_{4}=k_1^2 \, , \quad z_{5}=\left(k_1-k_2\right){}^2 \, .
%\label{eq:bubble-box-propagators}
%\end{align}
%\begin{align}
%z_{1} &= (k_2{-}p_1{-}p_2{-}p_3)^2 \, , \quad & z_{2} &= (k_2{-}p_2{-}p_3)^2  \, ,\nonumber\\
%z_{3} &= (k_2{-}p_3)^2  \, , \quad z_{4} = k_1^2 \, , \!\! & z_{5} &= (k_1{-}k_2)^2 \, .
%\label{eq:bubble-box-propagators}
%\end{align}
%Additionally we define the ISP
%\begin{equation}
%z_{6} = k_2{}^2.
%\label{eq:bbisp}
%\end{equation}
Within the \lbl BR~\cite{Frellesvig:2017aai}, $u$ reads:
\begin{align}
& u(\mathbf{z}) = \mathcal{B}_1^{\frac{2-d}{2}} \mathcal{B}_2^{\frac{d-3}{2}} \mathcal{B}_3^{\frac{d-5}{2}} \, ,
\end{align}
where
\begin{align}
%    B_1 &= z_6 \, , \quad B_2 = 2 \left(z_5+z_6\right) z_4 - z_4^2 - \left(z_5-z_6\right){}^2 \, ,\nonumber\\
%   B_2 = & s^2 z_2^2-2 t z_1 \left(z_3 (2 s+t)+s \left(t-z_2-z_6\right)\right)+\left(s\left(z_6\right.\right. \nonumber \\
%   & \left.-t\right)\left.+t z_3\right){}^2-2 s z_2 \left(z_6 (s+2 t)+s t-t z_3\right)+t^2 z_1^2 \, .
\mathcal{B}_1 &= z_6 \, , \quad \mathcal{B}_2 = 2 (z_5{+}z_6) z_4 - z_4^2 - (z_5{-}z_6)^2 \, ,\nonumber\\
\mathcal{B}_3 &= t^2 z_1^2 + s^2 z_2^2 - 2 t z_1 ((2 s {+} t) z_3 {+} s (t {-} z_2 {-} z_6)) \\ 
& \;\;\; - 2 s z_2 (s t {-} t z_3 {+} (s {+} 2 t) z_6) + (t z_3 {+} s (z_6 {-} t))^2.\nonumber
\end{align}
For all the possible $31 \, (=2^5{-}1)$ sectors, using eq.~\eqref{eq:criticalpoints} on the corresponding cut, we determine the number $N_{\text{sector}}$ of MIs. The non-zero cases are: $N_{1,2,3,4,5}=1$, $N_{1,3,4,5}=1$ and $N_{2,4,5}=1$, giving $3$ MIs. We choose them as:
\begin{equation}
J_1=\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box.png} \end{gathered} \, , \quad
J_2=\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{triangle_bubble.png} \end{gathered} \, , \quad
J_3=\begin{gathered} \includegraphics[width=0.03\textwidth,valign=c]{sunrise.png} \end{gathered} \, .
\end{equation}
Any integral $I$ of the form of eq.~\eqref{eq:def:I:basic}, with $u$ given in eq.~\eqref{eq:def:u:box}, and $\varphi$ defined in eq.~\eqref{eq:def:phi:FeynInt} (with $n=6$), can be decomposed as,
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_bump.png} \end{gathered}= c_1 \begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box.png} \end{gathered}+ c_2 \begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{triangle_bubble.png} \end{gathered}+ c_3\, \begin{gathered} \includegraphics[width=0.03\textwidth,valign=c]{sunrise.png} \end{gathered} \ . 
\label{eq:bubblebox:decomp}
\end{equation}
We use the set of spanning cuts ($\text{Cut}_{\{1,3,4,5\}}$, $\text{Cut}_{\{2,4,5\}}$) to obtain the full decomposition.\\
\noindent
$\bullet$ {$\rm \bf Cut_{\{1,3,4,5\}} : $}
On this specific cut, we use the regularized $u_{1,3,4,5}=z_2^{\rho_2} \, u(0,z_2,0,0,0;z_6)$ to obtain the corresponding $\hat{\omega}_2$ and $\hat{\omega}_6$. After choosing the $z_2$-coordinate for the inner space, using eq.~\eqref{eq:criticalpoints}, we get $\nu_{(62)}=2$, and $\nu_{(2)}=2$. We choose the basis forms as:
\begin{equation}
\hat{e}^{(62)}_{1}=\hat{h}^{(62)}_{1}=\frac{1}{z_2} \, , \qquad
\hat{e}^{(62)}_{2}=\hat{h}^{(62)}_{2}=1 \, ,
\end{equation}
and
\begin{equation}
\hat{e}^{(2)}_{1}=\hat{h}^{(2)}_{1}=\frac{1}{z_2} \, , \qquad
\hat{e}^{(2)}_{2}=\hat{h}^{(2)}_{2}=1 \, .
\end{equation}
$\bullet$ {$\rm \bf Cut_{\{2,4,5\}} : $}
On this cut, we use the regularized $u_{2,4,5}=z_1^{\rho_1}z_3^{\rho_3}u(z_1,0,z_3,0,0;z_6)$
to obtain the corresponding $\hat\omega_1$, $\hat\omega_3$ and $\hat\omega_6$. Using eq.~\eqref{eq:criticalpoints} we get $\nu_{(631)}=2$, $\nu_{(31)}=2$ and $\nu_{(1)}=2$. The basis forms are chosen as:
\begin{align}
\hat{e}^{(631)}_{1}&=\hat{h}^{(631)}_{1}=\frac{1}{z_1 z_3}, \qquad
\hat{e}^{(631)}_{2}=\hat{h}^{(631)}_{2}=1 \, ,
\nonumber \\
\hat{e}^{(31)}_{1}&=\hat{h}^{(31)}_{1}=z_1, \qquad
\hat{e}^{(31)}_{2}=\hat{h}^{(31)}_{2}=1,
\end{align}
and
\begin{equation}
\hat{e}^{(1)}_{1}=\hat{h}^{(1)}_{1}=z_1, \quad
\hat{e}^{(1)}_{2}=\hat{h}^{(1)}_{2}=1.
\end{equation}
Now, with the help of eq.~\eqref{eq:masterdeco} and using eq.~\eqref{eq:multivarIntNumb} for 
the computation the individual multi-variate (here 2 and 3-forms) intersection numbers, we 
determine the coefficients $c_i$ in eq.~\eqref{eq:bubblebox:decomp}.\\
\noindent
\textbf{Example. } Let us consider the decomposition of 
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_dotted.png} \end{gathered}=\int_{\mathcal{C}} \frac{u \,  d^6 \mathbf{z}}{z_1 z_2^2 z_3 z_4 z_5 }.
\end{equation}
On the $\text{Cut}_{1,3,4,5} $, we obtain:
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_dotted_cut.png} \end{gathered}=\int_{\mathcal{C}} u_{1,3,4,5} \, \varphi_{1,3,4,5} \, , \quad \varphi_{1,3,4,5}=\hat{\varphi}_{1,3,4,5} dz_2 \wedge dz_6
\end{equation}
where $\hat{\varphi}_{1,3,4,5}=\frac{\hat{\omega}_2}{z_2}$. 
%and $f_2=\frac{1}{u} \frac{\partial u}{\partial z_2}$. 
On this specific cut, we have:
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_dotted_cut.png} \end{gathered}=c_1 \begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_cut.png} \end{gathered}+c_2
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{triangle_bubble_cut.png} \end{gathered} \, ,
\end{equation}
with:
\begin{align}
c_1 & = \sum_{j=1}^{2} \langle \varphi_{1,3,4,5} | h_j^{(62)} \rangle \big({\mathbf C}_{(62)}^{-1}\big)_{j1} \nonumber \\
& = -\frac{3 (d-4) (2 (d-4) s+(d-2) t)}{2 (d-6) s t} \, ,\\
c_2 & = \sum_{j=1}^{2} \langle \varphi_{1,3,4,5} | h_j^{(62)} \rangle \big({\mathbf C}_{(62)}^{-1}\big)_{j2}
= -\frac{3 (d-4) (3 d-10)}{2 (d-6) s t} \, .\nonumber
\end{align}
On the $\text{Cut}_{2,4,5} $, we obtain:
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_dotted_cut2.png} \end{gathered}
=\int_{\mathcal{C}} u_{2,4,5} \, \varphi_{2,4,5} \, , \quad \varphi_{2,4,5}=\hat{\varphi}_{2,4,5} \, dz_1 \wedge dz_3 \wedge dz_6 \, ,
\end{equation}
where $\hat{\varphi}_{2,4,5}=\frac{\hat{\omega}_2}{z_1 z_3}$.
%and $f_2=\frac{1}{u} \frac{\partial u}{\partial z_2}$. 
On this specific cut, we have:
\begin{equation}
\begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_dotted_cut2.png} \end{gathered}=c_1 \begin{gathered} \includegraphics[width=0.05\textwidth,valign=c]{bubble_box_cut2.png} \end{gathered}+c_3 \begin{gathered}
\includegraphics[width=0.05\textwidth,valign=c]{sunrise_cut.png} \ ,
\end{gathered}
\end{equation}
where $c_1$ is in agreement with the value found on the $\text{Cut}_{1,3,4,5}$, and 
\begin{align}
%c_1 & = \sum_{j=1}^{2} \langle \varphi_{2,4,5} | h_j^{(631)} \rangle \big(\big({\mathbf C}^{(631)}\big)^{-1}\big)_{j1} \nonumber \\
%&= -\frac{3 (d-4) (2 (d-4) s+(d-2) t)}{2 (d-6) s t},\\
c_3 & = \sum_{j=1}^{2} \langle \varphi_{2,4,5} | h_j^{(631)} \rangle \big({\mathbf C}_{(631)}^{-1}\big)_{j2} \nonumber \\
& = \frac{3 (d-2) (3 d-10) (3 d-8)}{2 (d-6)^2 s t^2} \ .
\end{align}
Finally, we obtain a relation of the same type as in eq.~\eqref{eq:bubblebox:decomp}, in agreement with the IBP decomposition.






% Let us consider the reduction to master integral of the following integral: 
% \begin{align}
%     I_{1,2,1,1,1;0} = & \int_{\mathcal{C}} \frac{u}{z_1 \, z_2^2 \, z_3 \, z_4 \, z_5} \\
%     = & \int_{\mathcal{C}} \frac{\phi \, u}{z_1 \, z_2 \, z_3 \, z_4 \, z_5}
% \end{align}
% with
% \begin{equation}
%     \phi = \frac{\partial \log u}{\partial z_2} \, .
% \end{equation}
% Applying the Lee Pomeransky criterion on each possible cut of $u$, we are able to determine which sectors contain masters. In this case we choose as a master integral basis
% \begin{align}
%     & J_1 = I_{1,1,1,1,1;0} = \langle e_1 | \mathcal{C} ]  \, , \quad  J_2= I_{1,0,1,1,1;0} = \langle e_2 | \mathcal{C} ] \, , \nonumber \\
%      &  \quad \quad \quad \quad \quad J_3= I_{0,1,0,1,1;0} = \langle e_3 | \mathcal{C} ] \, \ .
% \end{align}

% %\subsection{Maximal cut}
% %On the maximal cut, we have
% %\begin{align}
% %& u = z_6^{\frac{d}{2}-2} \left(z_6-t\right)^{d-5} , \,
% %\omega =
% %\bigg(-\frac{-d t+3 d z_6+4 t-14 z_6}{2 z_6 \left(t-z_6\right)} 
% %\bigg) dz_6 
% %\, , \\
% %& \masters=1 \, , \hspace{3.25cm} \mathcal{P}=\{ 0 \,,\; t\,,\; \infty \} \, ,
% %\end{align}
% %with $\masters$ the number of critical points of $u$, obtained solving 
% %\begin{equation}
% %    \omega=0 \, .
% %\end{equation}
% %The form that corresponds to the integral we want to reduce reads
% %\begin{equation}
% %    \bra{\phi}=-\frac{(d-5) \left(s \left(t+z_6\right)+2 t z_6\right)}{s \left(z_6-t\right){}^2} \, dz_6
% %\end{equation}
% %Here the only master integral that is non-zero is
% %\begin{align}
% %    J_1= I_{1,1,1,1,1;0} = \langle e_1 | \mathcal{C} ] \ .
% %\end{align}
% %with 
% %\begin{align}
% %  \bra{e_1}= dz_6 \, .
% %\end{align}
% %The decomposition of $I_{1,2,1,1,1;0} = \langle \phi | \cal{C} ]$ in terms of $J_1$ reads
% %\begin{align}
% %\langle \phi | = \langle \phi | e_1 \rangle \,\textbf{C}_{11}^{-1}\, \langle e_1|.
% %\label{eq:2LBB:GD}
% %\end{align}
% %We build the metric matrix \textbf{C}, which has a single entry in this case.
% %\begin{align}
% %\textbf{C} =  \langle e_1 | e_1 \rangle  = \frac{4 \left(d t^2-5 t^2\right)}{3 (3 d-16) (3 d-14)}.
% %\end{align}
% %In this case the $\textbf{C}^{-1}$ is trivial to compute as the \textbf{C} contains only one element.
% %The other necessary intersection number is the following.
% %\begin{align}
% %\langle \phi | e_1 \rangle &=-\frac{2 (d-5) (d-4) t (2 (d-4) s+(d-2) t)}{(d-6) (3 d-16) (3 d-14) s} \ .
% %\end{align}
% %Using these in eq.~(\ref{eq:2LBB:GD}) we obtain the following reduction formula on the maximal cut
% %\begin{align}\label{massless-bubblebox-result}
% %I_{1,2,1,1,1;0} = -\frac{3 (d-4) (2 d s+d t-8 s-2 t)}{2 (d-6) s t} I_{1,1,1,1,1;0},
% %\end{align}
% %which agrees with the \textsc{Reduze 2}. \\

% \subsection{Next to maximal cut}
% The only interesting next-to-maximal cut is the cut which sets $z_1=z_3=z_4=z_5=0$, because all other possible combination would leads to sectors which does not contain any master.
% On the cut above mentioned we have
% \begin{align}
% u  =  z_2^{\beta} & z_6^{\frac{d}{2}-2} \left(s \left(t^2-2 t \left(z_2+z_6\right)+\left(z_2-z_6\right){}^2\right)-4 t z_2 z_6\right){}^{\frac{d-5}{2}} \\
% \hat{\omega}_{z_2} = &% \frac{\partial \log u}{\partial z_2} = 
% %\bigg(
% \frac{\beta}{z_2}-\frac{(d-5) \left(s \left(t-z_2+z_6\right)+2 t z_6\right)}{s \left(t^2-2 t \left(z_2+z_6\right)+\left(z_2-z_6\right){}^2\right)-4 t z_2 z_6}%-\frac{(d-5) \left(z_6 (s+2 t)+s t-s z_2\right)}{-2 z_2 \left(z_6 (s+2 t)+s t\right)+s \left(t-z_6\right){}^2+s z_2^2}
% %\bigg) dz_2 
% \, , \\
% \hat{\omega}_{z_6}  = &%\frac{\partial \log u}{\partial z_6} \\
% % = &\bigg(
% \frac{d-4}{2 z_6} -\frac{(d-5) \left(s \left(t+z_2-z_6\right)+2 t z_2\right)}{s \left(t^2-2 t \left(z_2+z_6\right)+\left(z_2-z_6\right){}^2\right)-4 t z_2 z_6}
% %\bigg) dz_6
% \, , \\
% \masters  = & 2 \, .
% \end{align}
% with $\masters$ the number of critical points of $u$, obtained solving 
% \begin{equation}
%     \begin{cases} \hat{\omega}_{z_2}=0 \\ \hat{\omega}_{z_6}=0 \end{cases} 
% \end{equation}
% The function %form
% that corresponds to the integral we want to reduce reads
% \begin{equation}
%      \bra{\phi}
%      %\hat{\phi}
%      =-\frac{(d-5) \left(s \left(t-z_2+z_6\right)+2 t z_6\right)}{s \left(t^2-2 t \left(z_2+z_6\right)+\left(z_2-z_6\right){}^2\right)-4 t z_2 z_6} \, dz_2 \wedge dz_6
% \end{equation}
% In this case the non-zero master integrals are
% \begin{align}
%     J_1= I_{1,1,1,1,1;0} = \langle e_1 | \mathcal{C} ] \, , \quad J_2= I_{1,0,1,1,1;0} = \langle e_2 | \mathcal{C} ] 
% \end{align}
% with 
% \begin{align}
%   \bra{e_1}=\frac{dz_2 \wedge dz_6}{z_2} \, , \quad \bra{e_2}= dz_2 \wedge dz_6 \, , \\
% \end{align}
% %The decomposition of $I_{1,2,1,1,1;0} = \langle \phi | \cal{C} ]$ in terms of $J_1$ and $J_2$ reads
% %\begin{align}
% %\langle \phi | = \sum_{i,j = 1}^{2} \langle \phi |e_j \rangle 
% %\left( \textbf{C}^{-1}\right)_{ji} \langle e_i|.
% %\label{eq:BB-nexttomaximalcut:GD}
% %\end{align}
% %
% %We compute the $\mathbf{C}$ matrix:
% %\begin{equation}
% %\mathbf{C}_{ij}=\bra{e_{i}}\ket{e_{j}} \, , \quad i,j=1,2;
% %\end{equation}
% %%with:
% %\begin{align}
% %\bra{e_{1}}\ket{e_{1}}= & \frac{4 (d-5) t ((d-4) t-2 \beta  (s+t))}{\beta  %(2 (\beta -8)+3 d) (2 (\beta -7)+3 d) (2 (\beta -6)+3 d)} \, , \\
% %\bra{e_{1}}\ket{e_{2}}= & \frac{8 (d-5) s t (2 s (\beta +d-5)+t (2 \beta +d-6))}{(2 (\beta -9)+3 d) (2 (\beta -8)+3 d) (2 (\beta -7)+3 d) (2 (\beta -6)+3 d)} \, , \\
% %\bra{e_{2}}\ket{e_{1}}= & \frac{8 (d-5) s t ((d-4) (2 s+t)+2 \beta  (s+t))}{(2 (\beta -8)+3 d) (2 (\beta -7)+3 d) (2 (\beta -6)+3 d) (2 (\beta -5)+3 d)} \, , \\
% %\bra{e_{2}}\ket{e_{2}}=& -\frac{16 (d-5) s^2 t \left(t \left(2 (\beta -7) \beta +2 d^2+3 (\beta -6) d+40\right)+2 s (\beta +d-5) (\beta +d-4)\right)}{(2 (\beta -9)+3 d) (2 (\beta -8)+3 d) (2 (\beta -7)+3 d) (2 (\beta -6)+3 d) (2 (\beta -5)+3 d)} \, .
% %\end{align}
% %The other necessary intersection numbers read: 
% %\begin{align}
% %\bra{\phi}\ket{e_{1}}= & \frac{2 (d-5) t \left(2 s \left(-2 \left(\beta ^2+\beta +8\right)-d^2+(\beta +8) d\right)-t (d-2 (\beta +1)) (d-2 (\beta +2))\right)}{\beta  s (2 (\beta -8)+3 d) (2 (\beta -7)+3 d) (2 \beta +d-6)} \, , \\
% %\bra{\phi}\ket{e_{2}}= & -\frac{4 (d-5) t ((d-2) t-2 \beta  (s+t)+2 s)}{(2 (\beta -9)+3 d) (2 (\beta -8)+3 d) (2 (\beta -7)+3 d)}  \, .
% %\end{align}
% Using then eq.~\eqref{eq:masterdeco} we obtain the reduction
% \begin{equation}
% I_{1,2,1,1,1;0}= c_{1} \, J_{1} + c_{2} \, J_{2} \, ,
% \end{equation}
% where,
% \begin{equation}
% \begin{split}
% & c_{1}= -\frac{(2 (\beta -6)+3 d) (2 s (\beta +d-4)+t (d-2 (\beta +1)))}{2 s t (2 \beta +d-6)} \, , \\
% & c_{2}=-\frac{(2 (\beta -6)+3 d) (2 (\beta -5)+3 d)}{2 s t (2 \beta +d-6)} \, ,
% \end{split}
% \end{equation}
% which, in the limit of $\beta \xrightarrow{} 0$ gives
% \begin{equation}
% \begin{split}
% & c_{1}=-\frac{3 (d-4) (2 (d-4) s+(d-2) t)}{2 (d-6) s t} \, , \\
% & c_{2}=-\frac{3 (d-4) (3 d-10)}{2 (d-6) s t} \, ,
% \end{split}
% \end{equation}
% in agreement with {\sc Reduze 2}. 

% \subsection{Triple cut}
% The only interesting triple cut is the cut which sets $z_2=z_4=z_5=0$, because all other possible combination would leads to sectors which does not contain any master.
% On the cut above mentioned we have
% \begin{align}
% u = & z_1^{\beta } z_3^{\rho} z_6^{\frac{d}{2}-2} \left(-2 t z_1 \left(s \left(t+2 z_3-z_6\right)+t z_3\right)\right. \\
% &\left.+\left(s \left(z_6-t\right)+t z_3\right){}^2+t^2 z_1^2\right){}^{\frac{d-5}{2}}\\
% \hat{\omega}_{z_1} = & \frac{\partial \log u}{\partial z_1} \, , \quad \hat{\omega}_{z_3} =  \frac{\partial \log u}{\partial z_3} \, , \quad \hat{\omega}_{z_6} =  \frac{\partial \log u}{\partial z_6} %= \bigg(
% %\frac{(5-d) t \left(-z_3 (2 s+t)+s \left(z_6-t\right)+t z_1\right)}{t^2 z_1^2-2 t z_1 \left(z_3 (2 s+t)+s \left(t-z_6\right)\right)+\left(s \left(z_6-t\right)+t z_3\right){}^2}+\frac{\beta}{z_1}
% %\bigg) dz_1 
% \, , \\
% %\hat{\omega}_{z_3} = & \frac{\partial \log u}{\partial z_3}% = \bigg(
% %\frac{\rho}{z_3}-\frac{(d-5) t \left(z_1 (2 s+t)+s \left(t-z_6\right)-t z_3\right)}{-2 t z_1 \left(z_3 (2 s+t)+s \left(t-z_6\right)\right)+\left(s \left(z_6-t\right)+t z_3\right){}^2+t^2 z_1^2}
% %\bigg) dz_3 
% %\, , \\
% %\hat{\omega}_{z_6} = & \frac{\partial \log u}{\partial z_6} %\\
% %= & \bigg(
% %\frac{-2 t z_1 \left((d-4) z_3 (2 s+t)+(d-4) s t+(9-2 d) s z_6\right)}{2 z_6 \left(-2 t
%   %z_1 \left(z_3 (2 s+t)+s \left(t-z_6\right)\right)+\left(s \left(z_6-t\right)+t z_3\right){}^2+t^2 z_1^2\right)} + \\
%   % & +\frac{\left(s \left(t-z_6\right)-t z_3\right) \left((d-4) t \left(s-z_3\right)+(14-3 d) s z_6\right)+(d-4) t^2 z_1^2}{2 z_6 \left(-2 t
%   % z_1 \left(z_3 (2 s+t)+s \left(t-z_6\right)\right)+\left(s \left(z_6-t\right)+t z_3\right){}^2+t^2 z_1^2\right)}%\bigg) dz_6
% %\, , \\
% \masters = & 2 \, .
% \end{align}
% with $\masters$ the number of critical points of $u$, obtained solving 
% \begin{equation}
%     \begin{cases} \hat{\omega}_{z_1}=0 \\ \hat{\omega}_{z_3}=0 \\ \hat{\omega}_{z_6}=0 \end{cases} 
% \end{equation}
% The form that corresponds to the integral we want to reduce reads
% \begin{equation}
%     \bra{\phi}=-\frac{(d-5) s \left(s \left(t+z_6\right)-t \left(z_1+z_3\right)+2 t z_6\right)}{-2 t z_1 \left(z_3 (2 s+t)+s \left(t-z_6\right)\right)+\left(s \left(z_6-t\right)+t z_3\right){}^2+t^2 z_1^2} \, dz_1 \wedge dz_3 \wedge dz_6
% \end{equation}
% In this case the non-zero master integrals are
% \begin{align}
%     J_1= I_{1,1,1,1,1;0} = \langle e_1 | \mathcal{C} ] \, , \quad J_3= I_{0,1,0,1,1;0} = \langle e_3 | \mathcal{C} ] \ .
% \end{align}
% with 
% \begin{align}
%   & \bra{e_1}=\frac{dz_1 \wedge dz_3 \wedge dz_6}{z_1 \, z_3} \, , \\
%   & \bra{e_3}= dz_1 \wedge dz_3 \wedge dz_6 \, , \\
% \end{align}
% %The decomposition of $I_{1,2,1,1,1;0} = \langle \phi | \cal{C} ]$ in terms of $J_1$ and $J_3$ reads
% %\begin{align}
% %\langle \phi | = \sum_{i,j = 1}^{2} \langle \phi |e_j \rangle 
% %\left( \textbf{C}^{-1}\right)_{ji} \langle e_i|.
% %\label{eq:BB-triplecut:GD}
% %\end{align}
% %
% %which leads to
% Using then eq.~\eqref{eq:masterdeco} we obtain the reduction
% \begin{equation}
% I_{1,2,1,1,1;0}= c_{1} \, J_{1} + c_{3} \, J_{3} \, ,
% \end{equation}
% where, after taking the limit of $\beta \rightarrow 0$ and $\rho \rightarrow 0$, we have
% \begin{equation}
% \begin{split}
% & c_{1}=-\frac{3 (d-4) (2 (d-4) s+(d-2) t)}{2 (d-6) s t} \, , \\
% & c_{3}= \frac{3 (d-2) (3 d-10) (3 d-8)}{2 (d-6)^2 s t^2} \, ,
% \end{split}
% \end{equation}
% in agreement with {\sc Reduze 2}. 



